Inference for high-dimensional instrumental variables regression

This paper concerns statistical inference for the components of a high-dimensional regression parameter despite possible endogeneity of each regressor. Given a first-stage linear model for the endogenous regressors and a second-stage linear model for the dependent variable, we develop a novel adaptation of the parametric one-step update to a generic second-stage estimator. We provide conditions under which the scaled update is asymptotically normal. We then introduce a two-stage Lasso procedure and show that the second-stage Lasso estimator satisfies the aforementioned conditions. Using these results, we construct asymptotically valid confidence intervals for the components of the second-stage regression coefficients. We complement our asymptotic theory with simulation studies, which demonstrate the performance of our method in finite samples.

==> estimation/bounds/ep.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Empirical process terms}\label{ep}

Theorem \ref{thm:oracle} provides a deterministic guarantee for the $\ell_1$ estimation error of a generic Lasso estimator $\gregh$ on the set $\gT(\tune) = \bset{4\|\gX^\top\gerr/n\|_\infty \le \tune}$.
Consequently, it holds that
\begin{align*}
  \Prb\bset{\|\gregh-\greg\|_1 > 4\gs\tune^2/\gcc^2}
  \smallpad\le
  \Prb\,\gT(\tune)^\comp \,.
\end{align*}
The quantity $\|\gX^\top\gerr/n\|_\infty$ is sometimes called the \emph{empirical process term}; for instance, \cite[Chapter 6]{BvdG11}.

It follows from the previous display that upper bounds for
$\Prb\,\gT(\tune)^\comp$ yield probabilistic guarantees for the $\ell_1$ estimation error.
We present such bounds for the first- and second- stages in Sections \ref{first} and \ref{second}, respectively.

\renewcommand{\gs}{\sigma}

We pause to recognize and abbreviate a genre of quantities that we will encounter frequently.
Define
\be\label{znM}
	\maxzn{\aM} \smallpad{:=} \|\dZ^\top\aM/n\|_\infty
\ee
for a given array $\aM=(\am_1,\ldots,\am_p)\in\R^{p\times n}$, including cases in which $p=1$; for instance, $\aM=\du$.
We also adopt the convention that $\maxzzn :=\maxzn{\dZ}=\|\rSzh\|_\infty$.

The following lemma is used throughout our consideration of the Gaussian error regime via the subsequent corollaries.
We present the bound in terms of a generic Gaussian vector~$\gauss$.

\begin{lem}[Control of $\maxzn{\gauss}$, Gaussian noise]\label{lem:epg} % Empirical Process, Gaussian
Let $\gauss\,|\,\dZ \sim \Normal_{n}(\bs{0}, \tau^2\Id)$. Then,
\benn
\begin{split}
	\Prb\big\{4\|\dZ^\top\gauss/n\|_\infty >
		\tau c \sqrt{\maxzzn\log\pz/\n}\big\}
  \relates{\le} 2\pz^{-\cepg}\,,
\end{split}
% \quad
% \begin{split}
%   \cepg \relates{:=} \frac{c^2}{32} - 1\,,
% \end{split}
\eenn
where $\cepg = c^2/32 - 1$ and $c>0$ is a controlled constant.
\end{lem}

%%%%%%%%%%
% PROOF
\myproof{Proof of Lemma \ref{lem:epg}}{%
The proof is similar to the treatments of \cite[Theorem 6]{JM14} and \cite[Lemma 6.2]{BvdG11}.
For each $j\in[\px]$, write $H_j := \ip{\dz^j,\gauss}/(\|\dz^j\|_2\tau)$.
It follows from the specification of $\gauss$ that $H_j \smallpad{|} \dz^j \sim \Normal(0,1)$.
Observe that
\begin{align*}
	& \Prb\big\{|\ip{\dz^j, \gauss}/n| > \tau \sqrt{\maxzzn(t^2 + 2\log\pz)/\n}\big\} \\
	\smallpad{&\qquad\le}
	\Prb\big\{|\ip{\dz^j,\gauss}/n| > \|\dz^j/\sqrt{n}\|_2 \tau \sqrt{(t^2 + 2\log\pz)/\n}\big\} \\
	\smallpad{&\qquad=}
	\Prb\big\{|H_j| > \sqrt{t^2 + 2\log\pz}\big\} \\
	\smallpad{&\qquad=}
	\E\big[\Prb\big\{|H_j| > \sqrt{t^2 + 2\log\pz}\smallpad{\big|} \dz^j\big\}
		\big] \\
	\smallpad{&\qquad=}
	\E\big[2\Prb\big\{H_j > \sqrt{t^2 + 2\log\pz}\smallpad{\big|} \dz^j\big\}
		\big] \\
	\smallpad{&\qquad\le}
	\E\big[2e^{-(t^2 + 2\log\pz)/2}\big] \smallpad= 2e^{-(t^2 + 2\log\pz)/2} \,,
\end{align*}
where the final line is just the Chernoff bound for $\Normal(0,1)$ random variables.
Take the union bound over $j\in[\px]$ to find
\begin{align*}
	& \Prb\Big\{\maxjpx|\ip{\dz^j, \du}/n| > \tau \sqrt{\maxzzn(t^2 + 2\log\pz)/\n}\Big\} \\
	\smallpad{&\qquad\le}
	2\px e^{-(t^2 + 2\log\pz)/2} \smallpad= 2e^{-t^2/2} \,.
\end{align*}
To conclude, choose $t$ so that $e^{t^2/2} = \pz^{\cepg}$ and observe that
\begin{align*}
	4\sqrt{(t^2+2\log\pz)/n}
	% \equals 4\sqrt{\log(\pz e^{t^2/2})/n}
	\aequals 4\tau\sqrt{2\log(\pz^{\cepg+1})/n} \\
	\aequals 4\tau\sqrt{(c^2/16)\log(\pz)/n}
	\equals \tau c\sqrt{\log\pz)/n} \,.
\end{align*}
}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}[Control of $\maxzn{\du}$, Gaussian noise]\label{lem:epu}
Suppose that $\du$ satisfies Assumption~\ref{assu:subgaussian}.
Define the set
\benn
	\Tu(\lambda)
	\smallpad{:=}
	\{\maxzn{\du} \leq \lambda\}
	\smallpad{=}
	\{\|\dZ^\top\du/\n\|_\infty \leq \lambda\} \,,
\eenn
where $\lambda$ is a controlled quantity.
Then
\benn
	\Prb\, \Tu\big(c \sdu \sqrt{\smash{\maxzzn}\log\pz/(2n)}\big)^\comp
	\smallpad\le
	2\pz^{-\cepg} \,.
\eenn
\end{lem}

%%%%%%%%%%
% PROOF

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{cor}[Control of $\maxzn{\dV}$, Gaussian noise]\label{epVg}
Suppose that $\dV$ satisfies Assumption~\ref{assu:subgaussian}.
Define the set
\begin{equation}\label{def:TV}
	\TV(\lambda)
	\smallpad{:=}
	\big\{\maxzn{\dV} \le \lambda\big\}
	\equals
	\big\{\|\dZ^\top\dV/\n\|_\infty \le \lambda\big\} \,,
\end{equation}
where $\lambda$ is a controlled quantity.
Then,
\benn
	\Prb \, \TV\big( c \maxsdv \sqrt{\smash{\maxzzn}\log\pz/(2n)}\big)^\comp
	\smallpad{\le}
	2\pz^{1-\cepg} \,,
\eenn
where $\cepg$ is as defined in Lemma \ref{lem:epg} and $\maxsdv = \maxjpx\sdvj$.
\end{cor}

%%%%%%%%%%
% PROOF
\myproof{Proof of Corollary \ref{epVg}}{%
Note that, for a given $\lambda$,
\begin{align*}
	\TV(\lambda)
	\equals
	\bigcap_{j\in[\px]} \bset{\|\dZ^\top\dv^j/\n\|_\infty \le \lambda} \,.
\end{align*}
Hence
\begin{align*}
	\Prb\,\TV\big(c \maxsdv \sqrt{\smash{\maxzzn}\log\pz/(2n)}\big)^\comp
	\smallpad{&=}
	\Prb\bigcup_{j\in[\px]} \bset{\|\dZ^\top\dv^j/n\|_\infty >
		c \maxsdv \sqrt{\smash{\maxzzn}\log\pz/(2n)}} \\
	\smallpad{&\le}
		\sum_{j\in[\px]} \Prb\bset{\|\dZ^\top\dv^j/n\|_\infty >
			c \sdvj \sqrt{\smash{\maxzzn}\log\pz/(2n)}} \\
	\smallpad{&\le}
		2\px\pz^{-\cepg} \smallpad\le 2\pz^{1-\cepg} \,,
\end{align*}
as claimed.
}%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}[Simultaneous control of $\maxzn{\dv^j}$, Gaussian noise]\label{lem:epfsg}
Suppose that $\dV$ satisfies Assumption~\ref{assu:subgaussian}.
For each $j\in[\px]$, define the set
\be\label{def:Tvj}
	\Tvj(\lambda_j)
	\smallpad{:=}
	\bset{4\|\dZ^\top\dv^j/n\|_\infty \le \lambda_j} \,.
	% \smallpad{=}
	% \big\{\|\dZ^\top\dV/n\|_\infty \le \maxjpx\tunej\big\}\,.
\ee
Define the set
\be\label{def:TA}
	\TA(\lambda_j)_{j\in[\px]}
	\smallpad{:=}
	\bigcap_{j\in[\px]}\Tvj(\lambda_j)
\ee
Then,
\benn
	\Prb\big\{\TA(\sdvj c \sqrt{\smash{\maxzzn}\log\pz/\n})_{j\in[\px]}\big\}^\comp
	% \Big(\bigcap_{j\in[\px]} \Tvj(\sdvj c \sqrt{\smash{\maxzzn}\log\pz/\n})\Big)^\comp
	\smallpad\le
	2\pz^{1-\cepg}\,,
\eenn
where $\cepg$ is as defined in Lemma \ref{lem:epg}.
\end{lem}

%%%%%%%%%%
% PROOF
\myproof{Proof of Lemma \ref{lem:epfsg}}{%
Note that
\begin{align*}
	& \,
	\Prb\Big\{\bigcap_{j\in[\px]} \Tvj(\sdvj c \sqrt{\smash{\maxzzn}\log\pz/\n})\Big\}^\comp \\
	\smallpad{=&}
	\Prb\Big\{
		\bigcup_{j\in[\px]} \big\{4\|\dZ^\top\dv^j/n\|_\infty > \sdvj c\sqrt{\smash{\maxzzn}\log\pz/\n}\big\}\Big\} \,.
\end{align*}
By Lemma \ref{lem:epg}, the union bound for the probability of the right-hand event above is $2\px\pz^{-\cepg}$.
The result follows from the assumption under the presently studied regime that $\px \leq \pz$.
}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{rek}
Remark about $\TA(\lambda_j)_{j\in J} \subseteq \TV(\max_{j\in J}\lambda_j)$.
\end{rek}


==> estimation/bounds/first.tex <==
\subsubsection{First stage}\label{first}
\myappendix{
\subsection{Materials required for Section~\ref{first}}\label{proofs:first}
}

% We present bounds for the first stage of the two-stage estimation procedure described in Section~\ref{ss:two-stage}.
The first stage is a high-dimensional multi-task regression problem.
Recall that the model for~$\dx^j$ is given by
\benn
	\dx^j \equals \dZ\ra^j + \dv^j\,,
\eenn
where~$\dv^j$ has nontrivial covariance with the noise~$\du$.
% Theorem \ref{thm:oracle} entails that, on the set
% \benn
% 	\Tvj(\tunej) \equals \set{\maxzn{\dv^j} \le \tunej} \,,
% \eenn
% it holds that
% \benn
% 	\|\rah^j-\ra^j\|_1 \smallpad\le 4\saj\tunej/\ccompj \,.
% \eenn
It suffices for our purposes to take a na\"ive approach to bounding the quantity~$\maxerrverbfs \equals \maxjpx\|\rah^j-\ra^j\|_1$.
That is, we simultaneously bound the estimation error of each individual task.
One could use a more complex approach such as~\cite{LWZ15} to treat different patterns of joint sparsity amongst the first-stage regression vectors.

We make the following assumption.

\begin{assu}[First-stage compatibility conditions]\label{assu:ccss}
For each active set~$\Saj=\supp\ra^j$ of the first-stage model, there exists a constant~$\ccompj^2 > 0$ such that~$\dZ$ satisfies the compatibility condition with respect to~$\Saj$ and~$\ccompj^2$.
We assume that the~$\n$-indexed sequences of such constants~$\ccompj^2$ are bounded strictly away from zero uniformly in~$\n$.
We write~$\ccompa^2:=\maxjpx\ccompj^2$.
\end{assu}

% \begin{rek}[Feasibility of Assumption~\ref{assu:ccss}]
\noindent As stated in Definition~\ref{def:cc}, whether~$\dZ$ satisfies the compatibility condition with respect to one active set~$\Sa_{j_1}$ does not bear directly on whether it satisfies the compatibility condition with respect to another active set~$\Sa_{j_2}$ for~$j_1,j_2\in[\px]$.
As such, it is non-trivial to assume that the compatibility condition as specified in Definition~\ref{def:cc} holds for each active set~$\Saj$ for~$j\in[\px]$ when~$\px$ tends to infinity.
However, the condition that~$\dZ$ satisfies the compatibility condition with respect to each active set~$\Saj$ is entailed by requiring that~$\kappa(s, c_0)$ of~\eqref{re} for~$s=\max_{j\in[\px]\saj}$ and~$c_0=3$ be bounded away from 0.
% a factor of $\sqrt{s}$ is required to negotiate between the $\ell_1$ norm denominator of the compatibility condition and the $\ell_2$ denominator of the restricted eigenvalue condition).
Thus, the discussion of \cite[Section 4]{BRT09} concerning the feasibility of their Assumption RE($s,c_0)$ applies as well to Assumption~\ref{assu:ccss}.
% \end{rek}

We will refer to the following specific choices of first-stage tuning parameters throughout the sequel.

\begin{defi}[First-stage tuning parameters]\label{tpss}
The following choices of the first-stage tuning parameters are appropriate for the sub-Gaussian noise regime of Assumption~\ref{assu:subgaussian}:
\benn
	\tunej\smallpad{:=}\tunejverb \,,
\eenn
where~$\tolj>0$ is a controlled quantity.
We let~$\tunefs := (\tune_1,\ldots,\tune_{\px})$ denote the tuple of first-stage tuning parameters, and we write
\benn
	\tunea \smallpad{:=} \maxjpx \tunej \equals \tuneVverb \,,
\eenn
where~$\tolV=\maxjpx\tolj$.
\end{defi}

\noindent The following lemma provides finite-sample guarantees for~$\maxerrfs$ under the choice of tuning parameters in Definition~\ref{tpss}.

% \begin{defi}[Generic tuning parameters, $\rAh$]\label{assu:tpgeneric}\
% \begin{enumerate}
% 	\item $\tunea = \maxjpx \tunej$, where $\tunej > 0$ for $j\in[\px]$ are arbitrary;
% \end{enumerate}
% \end{defi}
%
% \begin{defi}[Tuning parameters, $\rAh$, Gaussian noise]\label{assu:tpgaussian}\
% \begin{enumerate}
% 	\item $\tunej = \sdvj c \sqrt{\maxzzn\log\pz/\n}$ for each $j\in[\px]$;
% \end{enumerate}
% \end{defi}

% \begin{rek}[Tuning parameters]
% [Insert remark about possible redundancy between $\tunea$ and $\tuneV$.]
% \end{rek}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\myappendix{%
The following generic bound for~$\maxerrfs$ can be combined with concentration results for specific distributions of the first-stage noise elements.
We present it separately for the sake of modularity with respect to such assumptions.

\begin{lem}[Generic bound for~$\maxerrfs$]\label{lem:eefs} % Estimation Error, First-Stage
Suppose that Assumption~\ref{assu:ccss} holds.
For each~$j\in[\px]$ and~$\lambda<0$, let the sets~$\Tvj(\lambda)$ be as defined in Lemma~\ref{lem:epV}.
% \be\label{def:Tvj}
% 	\Tvj(\lambda)
% 	\smallpad{:=}
% 	\big\{4\|\dZ^\top\dv^j/n\|_\infty \leq \lambda\big\}\,.
% \ee
Then, on the set~$\bigcap_{j\in[\px]} \Tvj(\tunej)$,
\benn
	\maxerrfs
	\smallpad\le
	4\sa\tunea/\ccompa^2
	\equals
	4\scca\tunea \,,
\eenn
where~$\tunej$ is the tuning parameter for the respective first-stage Lasso problem,~$\tunea$ and~$\sa$ are as defined in Section~\ref{s:two-stage} and~$\ccompa$ is as defined in Section~\ref{first}.
\end{lem}
}%

%%%%%%%%%%
% PROOF
\myappendix{%
\begin{proof}[Proof of Lemma \ref{lem:eefs}]
For each~$j\in[\px]$, \cite[Theorem 6.1, Lemma 6.2]{BvdG11} entails that
\begin{align*}
	\Tvj(\tunej)
	\equals
	\big\{4\|\dZ^\top\dv^j/n\|_\infty \leq \tunej\big\}
	\smallpad{&\subseteq}
	\big\{\|\rah^j-\ra^j\|_1 \leq 4\saj\tunej/\ccompj^2\big\} \\
	\smallpad{&\subseteq}
		\big\{\|\rah^j-\ra^j\|_1 \leq 4\sa\tunea/\ccompa^2\big\}\,,
\end{align*}
where the latter containment follows by specification of~$\sa, \tunea,$ and~$\ccompa$.
Take intersections over~$j\in[\px]$ on both sides of the above display to conclude.
\end{proof}
}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}[Bound for $\maxerrfs$]\label{lem:eefsg}
Suppose that Assumptions~\ref{assu:ccss} and~\ref{assu:subgaussian} hold.
Set $\tunej$ according to Definition~\ref{tpss}.
Then,
\benn
	\Prb\bset{\maxerrfs > 4\scca\tuneVverb}
	\smallpad\le
	\prbepallvj\,,
\eenn
where~$\tolV$ is as specified in Definition~\ref{tpss} and~$\Choeff$ is as defined in Lemma~\ref{lem:epg}.
% Consequently, if $\sa = o(\sqrt{n/\log\pz})$, then $\maxerrfs = o_P(1)$.
\end{lem}

%%%%%%%%%%
% PROOF
\myappendix{
\begin{proof}[Proof of Lemma \ref{lem:eefsg}]
Lemma \ref{lem:eefs} entails that
\benn
	\Prb\{\maxerrfs > 4\sa\tunea/\ccompa^2\}
	\smallpad{\le}
	\Prb \Big\{\bigcap_{j\in[\px]} \Tvj(\tunej)\Big\}^\comp \,.
\eenn
% \begin{align*}
	% \Prb\{\maxerrfs > 4\sa\tunea/\ccompa^2\}
	% \smallpad{&\le}
	% \Prb \Big\{\bigcap_{j\in[\px]} \Tvj(\tunej)\Big\}^\comp \\
	% \smallpad{&\le}
	% 	\sum_{j\in[\px]}\Prb\,\Tvj(\tunej)^\comp \,.
	% \smallpad{&\le}
		% \px\Prb\bset{\sdvj c \sqrt{\maxzzn\log\pz/\n}} \,.
% \end{align*}

Apply the estimate of Lemma~\ref{lem:epV} for the right-hand side to conclude.
\end{proof}
}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{rek}[Choice of $c$]\label{remarkc}
% In order for Lemma~\ref{lem:eefsg} to entail asymptotic negligibility of~$\maxerrfs$, the controlled quantity~$c$ must be chosen so that~$\cepg>1$.
% In the sequel, we assume without further comment that such a choice has been made.
% \end{rek}

\noindent
Note that, in order to obtain a rate of convergence, we must choose each~$\tolj$ so that~$\min_{j\in[\px]}\tolj^2\Choeff/\sgnvj^2 - 2$ is bounded strictly away from zero.
Such a task may not be feasible in practice.
Our empirical results, which we present in Section~\ref{s:numerics}, suggest that cross-validated choices of the tuning parameters for the first- and second-stage Lasso estimators suffice for good behavior of the resultant updated estimator~$\rbdb$.
For the sake of our theory, we assume that such appropriate choices of~$\tolj$ have been made.
Given such an assumption, Lemma~\ref{lem:eefsg} entails that~$\maxerrfs=O_{\Prb}(\sa\sqrt{\log(\pz)/\n})$, essentially identical to the Lasso rate for single task regression problems.

% Assuming that~$\maxzzn=O_{\Prb}(1)$ and that~$\sdv,~\ccompa$ are bounded strictly away from zero and infinity uniformly in~$\n$,
% The condition that~$\maxzzn=O_{\Prb}(1)$ follows from tail bounds for~$\|\rSzh-\rSz\|_\infty$; such bounds can be derived under, say, a sub-Gaussianity assumption for the~$\dz_i$ according to the reasoning of Example~\ref{exa:wl}.

We are primarily interested in controlling the maximum estimation error~$\maxerrfs$ in order to establish bounds for the second-stage estimation error~$\|\rbla-\rb\|_1$ in the following section.


==> estimation/bounds/oracle.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Oracle inequality}\label{oracle}
\newcommand{\gX}{\bs{W}}
\newcommand{\gx}{\bs{w}}
\newcommand{\gy}{\bs{g}}
\newcommand{\greg}{\bs{\gamma}}
\newcommand{\gregh}{\hat{\greg}}
\newcommand{\gerr}{\bs{h}}
\newcommand{\gS}{S_{\greg}}
\newcommand{\gSc}{\gS^{\comp}}
\renewcommand{\gs}{s_{\greg}}
\newcommand{\gcc}{\phi_{\greg}}
\newcommand{\gT}{\mathcal{T}}

The following theorem is generic over both the first- and second-stage Lasso estimators.
As such, we present it in terms of a generic model that shares notation with neither the first- nor second- stage models described in Section~\ref{model} except for the number of observations $\n$.

\begin{thm}[Oracle inequality]\label{thm:oracle}
Consider the generic linear model
\benn
  \gy \equals \gX\greg + \gerr \,,
\eenn
where $\gy\in\R^{\n}$ is a vector of univariate responses, $\gX\in\R^{\n\times p}$ is a design matrix with rows $\gx_i$, $\greg\in\R^{\n}$ is a noise vector with arbitrary distribution.
Let $\gregh$ denote the Lasso estimator given by
\benn
  \gregh \smallpad\in
  \argmin_{\bs{a}\in\R^{p}} \big\{
    \|\gy - \gX\bs{a}\|_2^2/(2\n) + \tune \|\bs{a}\|_1
  \big\} \,.
\eenn
Let $\gS := \supp\greg$, and let $\gs := |\gS|$.
Suppose that $\gX\in\Ccomp(\gS,\gcc)$ for a $\gcc>0$.
Then, on the set
\be\label{soi}
  \gT(\tune) \smallpad{:=} \bset{4\|\gX^\top\gerr/n\|_\infty \le \tune} \,,
\ee
the bound
\benn
  \|\gX(\gregh-\greg)\|_2^2/n + \tune\|\gregh-\greg\|_1
  \smallpad{\leq}
  4\gs\tune^2/\gcc^2
\eenn
holds.
\end{thm}

%%%%%%%%%%
% PROOF
\myproof{Proof of Theorem \ref{thm:oracle}}{%
The proof is algebra. See Theorem 6.1 of \cite{BvdG11}.
%To begin, note that the specification of $\gregh$ in the statement of the present theorem entails that
%\benn
%	\|\gy - \gX \gregh\|_2^2 / n + \tune\|\gregh\|_1 \smallpad{\le} \|\gy - \gX \greg \|_2^2 / n + \tune \|\greg\|_1 \, .
%\eenn
%Substituting $\gX \greg + \gerr$ for $\gy$ yields
%\benn
%	\| \gX(\greg - \gregh) + \gerr \|_2^2/n + \tune\|\gregh\|_1 \smallpad{\le} \|\gerr\|_2^2/n + \tune\|\greg\|_1 \, .
%\eenn
%On the left-hand side of the above we have
%\begin{align*}
%	\| \gX(\greg - \gregh) + \gerr \|_2^2 \aequals\|\gX(\greg - \gregh)\|_2^2 + 2\langle\gX(\greg - \gregh)\,, \gerr\rangle + \|\gerr\|_2^2 \, ,
%\end{align*}
%where $\langle \cdot\,,\,\cdot \rangle$ denotes the standard inner product over Euclidean space.
%As the first term on the right-hand side above is squared, we may swap the order of $\greg$ and $\gregh$ therein.
%Combining the two displays above and simplifying then yields
%\benn
%	\big[\| \gX(\gregh - \greg) \|_2^2 + 2\langle\gX(\greg - \gregh)\,, \gerr\rangle\big]/n + \tune\|\gregh\|_1 \smallpad{\le}
%		\tune\|\greg\|_1 \, .
%\eenn
%Rearranging terms in the above display leads to the following \emph{basic inequality}:
%\be\label{ineq:basic}
%	\| \gX(\gregh - \greg) \|_2^2/n + \tune\|\gregh\|_1 \smallpad{\le}  2\iprod{\gX(\gregh - \greg)}{\gerr}/n + \tune\|\greg\|_1 \, .
%\ee
%Apply H\"{o}lder's inequality to the modulus of the first term on the right-hand side above to find
%\begin{align*}
%	2 \iprod{\gX(\gregh - \greg)}{\gerr}/n \ \smallpad{&\le}2 \|\gX^\top\gerr/n\|_\infty\|\gregh - \greg\|_1 \\
%	\smallpad{&\le}\foh\tune \|\gregh - \greg\|_1 \,,
%\end{align*}
%where the latter inference holds on the set $\gT(\tune)$.
%Substitute the above display into the basic inequality of \eqref{ineq:basic} and double the result to find that
%\benn
%	2\|\gX(\gregh - \greg)\|_2^2/n + 2 \tune\|\gregh\|_1 \smallpad{\le} \tune\|\gregh-\greg\|_1 + 2 \tune\|\greg\|_1 \, .
%\eenn
%Now rearrange terms in the reverse triangle inequality
%\benn
%		\|(\gregh-\greg)_{\gS}\|_1 \equals \| \gregh_{\gS} - \greg_{\gS}\|_1 \smallpad{\ge} \|\greg_{\gS}\|_1 - \|\gregh_{\gS}\|_1
%\eenn
%to obtain that
%\benn
%	\|\gregh_{\gS}\|_1 \smallpad{\ge} \|\greg_{\gS}\|_1 - \|(\gregh-\greg)_{\gS}\|_1
%\eenn
%and hence that
%\begin{align*}
%	\| \gregh \|_1 \aequals\|\gregh_{\gS}\|_1 + \|\gregh_{\gSc}\|_1 \nonumber\\
%	& \geq \ \| \greg_{\gS} \|_1 - \| (\gregh-\greg)_{\gS} \|_1 + \|\gregh_{\gSc}\|_1 \, .
%\end{align*}
%Substitute the above display into the most recent derivation from the basic inequality to find
%\begin{align*}
%  & \ \,
%    2\|\gX(\gregh - \greg)\|_2^2 + 2r\big[ \| \greg_{\gS} \|_1 - \| (\gregh-\greg)_{\gS} \|_1 + \|\gregh_{\gSc}\|	_1 \big] \\
%  \le&\ \,
%    \tune\|\gregh-\greg\|_1 + 2\tune\|\greg\|_1 \\
%	=&\ \,
%    \tune\big[\|(\gregh - \greg)_{\gS}\|_1 + \|(\gregh - \greg)_{\gSc}\|_1\big] + 2\tune\big[\|\greg_{\gS}\|_1 + \|\greg_{\gSc}\| \big] \\
%	=& \ \,
%    \tune\big[\|(\gregh - \greg)_{\gS}\|_1 + \|\gregh_{\gSc}\|_1\big] + 2\tune\|\greg_{\gS}\|_1 \, ,
%\end{align*}
%where, to infer the final line, recall that $\|\greg_{\gSc}\|_1 = 0$ by specification of $\gS$.
%Simplify the above display by consolidating terms to find
%\benn
%	2\|\dX(\gregh-\greg)\|_2^2/n + \tune\|\gregh_{\gSc}\|_1 \smallpad{\le} 3\tune\|(\gregh-\greg)_{\gS}\|_1 \, .
%\eenn
%From the fact that the components of $\greg$ vanish on $\gS$ and from the decomposability of the $\ell_1$ norm, write
%\begin{align*}
%	\|\gregh_{\gSc}\|_1 \aequals\| (\gregh - \greg)_{\gSc}\|_1 \\
%	& = \ \| \gregh - \greg \|_1 - \| (\gregh - \greg)_{\gS}\|_1 \nonumber \, .
%\end{align*}
%Now substitute $\| \gregh - \greg \|_1 - \| (\gregh - \greg)_{\gS}\|_1$ for $\|\gregh_{\gSc}\|_1$ two displays previous and consolidate terms to obtain
%\benn
%	2\|\gX(\gregh-\greg)\|_2^2/n + \tune\|(\gregh-\greg)\|_1 \smallpad{\le} 4\tune\|(\gregh-\greg)_{\gS}\|_1 \, .
%\eenn
%Write
%\benn
%  \|(\gregh-\greg)\|_1 = \|(\gregh-\greg)_{\gS}\|_1 + \|(\gregh-\greg)_{\gSc}\|_1
%\eenn
%and combine with two displays previous to conclude that
%\benn
%	\| (\gregh - \greg)_{\gSc} \|_1 \smallpad{\le} 3 \| (\gregh - \greg)_{\gS} \|_1 \,.
%\eenn
%The above display is the hypothesis of the compatibility condition, which holds for $\gX$ relative to $\gS$ and $\gcc > 0$ by assumption.
%Invoke the compatibility condition to find
%\benn
%	\| (\gregh-\greg)_{\gS} \|_1 \smallpad{\le}  \sqrt{\gs} \|\gX(\gregh-\greg)\|_2 / (\sqrt{n}\gcc) \, .
%\eenn
%Next, write
%\begin{align*}
%	2\|\gX(\gregh-\greg)\|_2^2/n + \tune\|(\gregh-\greg)\|_1 \ \smallpad{&\le}4\tune  \sqrt{\gs} \|\gX(\gregh-\greg)\|_2 / (\sqrt{n}\gcc) \\
%	\smallpad{&\le}\|\gX(\gregh-\greg)\|_2^2/n + 4\gs\tune^2 / \gcc^2 \, ,
%\end{align*}
%where the last step follows from the inequality $4xy \leq x^2 + 4y^2$ for $x, y \in \R$.
%Subtract $\|\gX(\gregh - \greg)\|_2^2/n$ from both sides to find
%\benn
%	\| \gX(\gregh - \greg) \|_2^2 / n + \tune\|\gregh - \greg\|_1 \smallpad{\le} 4\gs\tune^2/\gcc^2 \, ,
%\eenn
%as claimed.
%}%

